Automatic BLAS Offloading on Unified Memory Architecture: A Study on NVIDIA Grace-Hopper

Porting codes to GPU often requires major efforts. While several tools exist for automatically offload numerical libraries such as BLAS and LAPACK, they often prove impractical due to the high cost of mandatory data transfer. The new unified memory architecture in NVIDIA Grace-Hopper allows high bandwidth cache-coherent memory access of all memory from both CPU and GPU, potentially eliminating bottleneck faced in conventional architecture. This breakthrough opens up new avenues for application development and porting strategies. In this study, we introduce a new tool for automatic BLAS offload, the tool leverages the high speed cache coherent NVLink C2C interconnect in Grace-Hopper, and enables performant GPU offload for BLAS heavy applications with no code changes or recompilation. The tool was tested on two quantum chemistry or physics codes, great performance benefits were observed.

==> rawdata.tex <==


PARSEC on H100 PCIE:  16x3 
dgemm time total= 200.080841, data=189.569999, compute=9.829369
data vol (GB): 751.955765, copy speed GB/s: 3.966639
dgemm time total= 269.764309, data=256.517730, compute=12.487587
data vol (GB): 1075.790167, copy speed GB/s: 4.193824
dgemm time total= 265.861231, data=252.850087, compute=12.306159
data vol (GB): 1076.086518, copy speed GB/s: 4.255828
dgemm time total= 200.400431, data=190.427680, compute=9.289868
data vol (GB): 750.189788, copy speed GB/s: 3.939500
dgemm time total= 263.825101, data=251.920554, compute=11.141736
data vol (GB): 1075.651864, copy speed GB/s: 4.269806
dgemm time total= 266.966219, data=254.531426, compute=11.675421
data vol (GB): 1073.998101, copy speed GB/s: 4.219511
dgemm time total= 199.982329, data=189.581050, compute=9.745207
data vol (GB): 753.372484, copy speed GB/s: 3.973881
dgemm time total= 200.902844, data=190.759805, compute=9.473226
data vol (GB): 750.855522, copy speed GB/s: 3.936131
dgemm time total= 201.296682, data=191.496250, compute=9.161006
data vol (GB): 749.742000, copy speed GB/s: 3.915179
dgemm time total= 201.649450, data=191.024531, compute=9.970306
data vol (GB): 753.031929, copy speed GB/s: 3.942069
dgemm time total= 266.721836, data=253.764357, compute=12.197538
data vol (GB): 1071.504936, copy speed GB/s: 4.222441
dgemm time total= 266.762511, data=254.258954, compute=11.747696
data vol (GB): 1072.743867, copy speed GB/s: 4.219100
dgemm time total= 266.181820, data=253.509298, compute=11.987563
data vol (GB): 1076.774489, copy speed GB/s: 4.247475
dgemm time total= 199.443446, data=189.094232, compute=9.774498
data vol (GB): 754.428889, copy speed GB/s: 3.989698
dgemm time total= 200.167184, data=190.101077, compute=9.428459
data vol (GB): 750.989243, copy speed GB/s: 3.950473
dgemm time total= 266.687605, data=254.290978, compute=11.628555
data vol (GB): 1076.226169, copy speed GB/s: 4.232263
----------
total vol:  14,613 GB
aggregated speed: 65.5GB/s

---------------dgemm----------------------- 
dgemm msize: 32 2400 93536, mmem: 1736.1 MiB
dgemm on gpu 1929.5
cudainit   time 0.000008
cudamalloc time 0.000007
cudamemcpy time 0.071081
cudablas1  time 0.001012
cudacpback time 0.000049
cudafree   time 0.000007
* my total time 0.072196
runtime(s)            0.072197
      # Result check     1870720.00   1870720
dgemm time total= 1.656823, data=1.423762, compute=0.225470
data vol (GB): 33.919983, copy speed GB/s: 23.824187

***with memcpyasync and cudaHostRegister
dgemm msize: 32 2400 93536, mmem: 1736.1 MiB
dgemm on gpu 1929.5
cudainit   time 0.000007
cudamalloc time 0.000004
cudamemcpy time 0.031746
cudablas1  time 0.000994
cudacpback time 0.000024
cudafree   time 0.000005
* my total time 0.032805
runtime(s)            0.032807
      # Result check     1870720.00   1870720
dgemm time total= 0.719542, data=0.635729, compute=0.036886
data vol (GB): 33.919983, copy speed GB/s: 53.356074


***************************

PAPRSEC on GH: 16x4
dgemm time total= 302.609441, data=284.771546, compute=11.654007
data vol (GB): 6992.829276, copy speed GB/s: 24.555927
dgemm time total= 272.046865, data=255.489399, compute=10.470714
data vol (GB): 5727.286859, copy speed GB/s: 22.416926
dgemm time total= 316.611837, data=298.016709, compute=12.662117
data vol (GB): 6991.465882, copy speed GB/s: 23.459979
dgemm time total= 304.678416, data=286.789441, compute=11.842563
data vol (GB): 6992.755737, copy speed GB/s: 24.382891
dgemm time total= 274.677946, data=257.263408, compute=11.294509
data vol (GB): 5729.436242, copy speed GB/s: 22.270700
dgemm time total= 275.991790, data=258.638767, compute=11.433016
data vol (GB): 5727.793821, copy speed GB/s: 22.145921
dgemm time total= 306.733039, data=288.002006, compute=12.630218
data vol (GB): 6990.517869, copy speed GB/s: 24.272462
dgemm time total= 307.185798, data=289.808819, compute=11.437851
data vol (GB): 6992.073641, copy speed GB/s: 24.126504
dgemm time total= 272.763503, data=255.507462, compute=11.144051
data vol (GB): 5730.047583, copy speed GB/s: 22.426146
dgemm time total= 313.577005, data=295.035530, compute=12.491333
data vol (GB): 6991.544016, copy speed GB/s: 23.697295
dgemm time total= 275.795887, data=258.248437, compute=11.528809
data vol (GB): 5728.832412, copy speed GB/s: 22.183416
dgemm time total= 312.265244, data=293.362210, compute=12.891981
data vol (GB): 6990.584186, copy speed GB/s: 23.829191
dgemm time total= 279.015028, data=261.865313, compute=11.173327
data vol (GB): 5728.762253, copy speed GB/s: 21.876751
dgemm time total= 311.235917, data=293.231144, compute=12.067380
data vol (GB): 6992.218347, copy speed GB/s: 23.845415
dgemm time total= 285.222596, data=267.342553, compute=11.793330
data vol (GB): 5728.237212, copy speed GB/s: 21.426582
dgemm time total= 274.083991, data=257.177227, compute=10.857414
data vol (GB): 5729.497076, copy speed GB/s: 22.278400
------- 
Total vol: 101,764 GB
aggregated speed: 369.2 GB/s


---------------dgemm----------------------- 
dgemm msize: 32 2400 93536, mmem: 1736.1 MiB
dgemm on gpu 1929.5
cudainit   time 0.000003
cudamalloc time 0.000002
cudamemcpy time 0.004861
cudablas1  time 0.000605
cudacpback time 0.000012
cudafree   time 0.000003
* my total time 0.005498
runtime(s)            0.005500
      # Result check      935360.00    935360
dgemm time total= 0.144597, data=0.049127, compute=0.014556
data vol (GB): 16.959991, copy speed GB/s: 345.226304





\textcolor{red}{
total vol:  14,613 GB
aggregated speed: 65.5GB/s
Total vol: 101,764 GB
aggregated speed: 369.2 GB/s
}
